SPIRE: Semantic Prompt-Driven Image Restoration

Text-driven diffusion models have become increasingly popular for various image editing tasks, including inpainting, stylization, and object replacement. However, it still remains an open research problem to adopt this language-vision paradigm for more fine-level image processing tasks, such as denoising, super-resolution, deblurring, and compression artifact removal. In this paper, we develop SPIRE, a Semantic and restoration Prompt-driven Image Restoration framework that leverages natural language as a user-friendly interface to control the image restoration process. We consider the capacity of prompt information in two dimensions. First, we use content-related prompts to enhance the semantic alignment, effectively alleviating identity ambiguity in the restoration outcomes. Second, our approach is the first framework that supports fine-level instruction through language-based quantitative specification of the restoration strength, without the need for explicit task-specific design. In addition, we introduce a novel fusion mechanism that augments the existing ControlNet architecture by learning to rescale the generative prior, thereby achieving better restoration fidelity. Our extensive experiments demonstrate the superior restoration performance of SPIRE compared to the state of the arts, alongside offering the flexibility of text-based control over the restoration effects.

==> sec/deprecated_2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/deprecated_3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/figs/content_prompt.tex <==
\begin{figure*}[t]
  \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth,height=0.4\linewidth]{example-image-golden}

   \caption{content prompt.}
   \label{fig:content prompt}
\end{figure*}

==> sec/figs/rebuttal/cfg_ablation.tex <==
\newcommand{\tuneimgwidth}{0.4\columnwidth}

% \begin{figure*}[!t]
% \centering
% % \footnotesize
% \setlength\tabcolsep{1pt}
% {
% \renewcommand{\arraystretch}{0.6}
% \resizebox{1\linewidth}{!}{
% \begin{tabular}{@{}*{7}{c}@{}}
%     \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/1_fox/input.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/1_fox/result_0_0_1115-0139.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/1_fox/result_0_3_1115-0139.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/1_fox/result_2_0_3_1115-0141.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/1_fox/result_3_0_3_1115-0141.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/1_fox/result_1_0_3_1115-0141.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/1_fox/gt.jpg}

%      \\ 

%     %  input & $\varnothing$=\emph{``''}, sample 1 & $\varnothing$=\emph{``''}, sample 2 & \emph{``Bichon Frise dog''} & \emph{``grey wolf''} & \emph{``white fox''} & Reference  \\

%      Input & \emph{``''}, sample 1 & \emph{``''}, sample 2 & \emph{``Bichon Frise dog''} & \emph{``grey wolf''} & \emph{``white fox''} & Reference  \\

%     \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/2_bear/input.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/2_bear/result_0_0_0_1115-0205.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/2_bear/result_0_0_1_1115-0205.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/2_bear/result_2_0_0_1115-0205.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/2_bear/result_3_0_1_1115-0205.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/2_bear/result_1_0_1_1115-0205.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/2_bear/gt.jpg}

%      \\ 

%      Input & \emph{ ``''}, sample 1 & \emph{``''}, sample 2 & \emph{``lion''} & \emph{`` tiger''} & \emph{``bear''} & Reference


%     %  input &  $\varnothing$=\emph{ ``''}, sample 1 & $\varnothing$=\emph{``''}, sample 2 & \emph{``lion''} & \emph{`` tiger''} & \emph{``bear''} & Reference 
    
% \end{tabular}
% }
% }
% \vspace{-1em}
% \caption{\textbf{Test-time semantic prompting}. Our framework restores degraded images guided by flexible semantic prompts, while unrelated background elements and global tones remain aligned with the degraded input conditioning.  }
% \label{fig:content_prompting}
% \vspace{-1em}
% \end{figure*}



\begin{figure}[h]
\centering
% \footnotesize
\setlength\tabcolsep{1pt}
{
\renewcommand{\arraystretch}{0.6}
\vspace{-0.35cm}
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}*{6}{c}@{}}
    \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/input.jpg} & 
    % \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/1_fox/result_0_0_1115-0139.jpg} & 
    \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/result_0_0_0.0_0_0126-1437.jpg} & 
    % \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/result_0_0_0.5_0_0126-1437.jpg} & 
    \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/result_0_0_1_0_0126-1437.jpg} & 
    \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/result_0_0_3.0_0_0126-1437.jpg} & 
    % \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/result_0_0_5.0_0_0126-1437.jpg} 
    % & 
    \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/result_0_0_7.5_0_0126-1437.jpg}

     \\ 

    %  input & $\varnothing$=\emph{``''}, sample 1 & $\varnothing$=\emph{``''}, sample 2 & \emph{``Bichon Frise dog''} & \emph{``grey wolf''} & \emph{``white fox''} & Reference  \\

     Input; $c_s=$``fox'' & \small{CFG=$0.0$ (same as $c_s=$``'')} & CFG=$1.0$ & CFG=$3.0$ & 
    %  CFG=$5.0$ &
     CFG=$7.5$  \\


    %  input &  $\varnothing$=\emph{ ``''}, sample 1 & $\varnothing$=\emph{``''}, sample 2 & \emph{``lion''} & \emph{`` tiger''} & \emph{``bear''} & Reference 
    
\end{tabular}
}
}
\vspace{-1em}
% \caption{\textbf{\todo{add figure}}.  }
% \label{fig:content_prompting}
% \vspace{-1em}
\end{figure}


==> sec/figs/rebuttal/face_restoration.tex <==
% \newcommand{\tuneimgwidth}{0.4\columnwidth}


\begin{figure}[h]
\centering
% \footnotesize
% \setlength\tabcolsep{1pt}
{

% \renewcommand{\arraystretch}{0.6}
\vspace{-0.35cm}
% \resizebox{1\linewidth}{!}{
% % \include{r1q1}
% \parbox{\imwidth}{
% \includegraphics[width=0.99\linewidth]{sec/figs/rebuttal/r1q1_face2.pdf}}
\includegraphics[width=0.77\linewidth]{sec/figs/rebuttal/ECCV_Rebuttal_2x3.pdf}}
\vspace{-0.2cm}
% \begin{tabular}{@{}*{6}{c}@{}}
%     \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/input.jpg} & 
%     % \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/1_fox/result_0_0_1115-0139.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/result_0_0_0.0_0_0126-1437.jpg} & 
%     % \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/result_0_0_0.5_0_0126-1437.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/result_0_0_1_0_0126-1437.jpg} & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/result_0_0_3.0_0_0126-1437.jpg} & 
%     % \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/result_0_0_5.0_0_0126-1437.jpg} 
%     % & 
%     \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/result_0_0_7.5_0_0126-1437.jpg}

%      \\ 

%     %  input & $\varnothing$=\emph{``''}, sample 1 & $\varnothing$=\emph{``''}, sample 2 & \emph{``Bichon Frise dog''} & \emph{``grey wolf''} & \emph{``white fox''} & Reference  \\

%      Input; $c_s=$``fox'' & \small{CFG=$0.0$ (same as $c_s=$``'')} & CFG=$1.0$ & CFG=$3.0$ & 
%     %  CFG=$5.0$ &
%      CFG=$7.5$  \\


%     %  input &  $\varnothing$=\emph{ ``''}, sample 1 & $\varnothing$=\emph{``''}, sample 2 & \emph{``lion''} & \emph{`` tiger''} & \emph{``bear''} & Reference 
    
% \end{tabular}
% }
% }
\vspace{-1em}
% \caption{\textbf{\todo{add figure}}.  }
% \label{fig:content_prompting}
% \vspace{-1em}
\end{figure}


==> sec/figs/rebuttal/multiple_object.tex <==


\begin{figure}[h]
\centering
% \footnotesize
\setlength\tabcolsep{1pt}
{
\renewcommand{\arraystretch}{0.6}
\vspace{-0.35cm}
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}*{4}{c}*{4}{c}@{}}
    \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/multi_object/input.jpg} & 
    % \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/1_fox/result_0_0_1115-0139.jpg} & 
    \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/multi_object/result_0_0_3_7.5__0126-1553.jpg} & 
    % \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/result_0_0_0.5_0_0126-1437.jpg} & 
    \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/multi_object/result_2_0_0_7.5_Zebra_0126-1553.jpg} & 
    \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/multi_object/result_3_0_3_7.5_Giraffe._0126-1553.jpg} & 
    \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/multi_object/result_9_0_3_7.5_giraffe and zebra grazing in a field next to plants._0126-1553.jpg}
    % \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/multi_object/gt.jpg}
     \\ 

    %  input & $\varnothing$=\emph{``''}, sample 1 & $\varnothing$=\emph{``''}, sample 2 & \emph{``Bichon Frise dog''} & \emph{``grey wolf''} & \emph{``white fox''} & Reference  \\

     Input & ``'' & ``Zebra'' & ``Giraffe'' & ``Giraffe and Zebra''  \\


    %  input &  $\varnothing$=\emph{ ``''}, sample 1 & $\varnothing$=\emph{``''}, sample 2 & \emph{``lion''} & \emph{`` tiger''} & \emph{``bear''} & Reference 
    
\end{tabular}
}
}
\vspace{-1.5em}
% \caption{\textbf{\todo{add figure}}.  }
% \label{fig:content_prompting}
% \vspace{-1em}
\end{figure}


==> sec/figs/rebuttal/realworld_example.tex <==
\begin{figure}[h]
\centering
% \footnotesize
\setlength\tabcolsep{1pt}
{
\renewcommand{\arraystretch}{0.6}
\vspace{-0.35cm}
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{\hspace{0mm}}*{4}{c}*{4}{c}@{\hspace{0mm}}}
    \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/real_images/lincoln_input.jpg} & 
    % \includegraphics[width=\tuneimgwidth]{sec/figs/sec4_exp/test_content_tuning/1_fox/result_0_0_1115-0139.jpg} & 
    \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/real_images/lincoln_result.jpg} & 
    % \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/semantic_cfg/result_0_0_0.5_0_0126-1437.jpg} & 
    \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/real_images/flower_input.jpg} & 
    \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/real_images/flower_result_3_0_3_7.5_0126-1522.jpg} & 
    
    % \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/real_images/51_512.jpg} & 
    % \includegraphics[width=\tuneimgwidth]{sec/figs/rebuttal/real_images/result_3_0_1_7.5_0126-1450.jpg}

     \\ 

    %  input & $\varnothing$=\emph{``''}, sample 1 & $\varnothing$=\emph{``''}, sample 2 & \emph{``Bichon Frise dog''} & \emph{``grey wolf''} & \emph{``white fox''} & Reference  \\

     Input & ``Lincoln'' & Input & ``Flower'' 
    %  & Input & ``Tower bridge''  
     
     \\


    %  input &  $\varnothing$=\emph{ ``''}, sample 1 & $\varnothing$=\emph{``''}, sample 2 & \emph{``lion''} & \emph{`` tiger''} & \emph{``bear''} & Reference 
    
\end{tabular}
}
}
\vspace{-1.2em}
% \caption{\textbf{\todo{add figure}}.  }
% \label{fig:content_prompting}
% \vspace{-1em}
\end{figure}


==> sec/figs/sec3_method/arbitrary_scale.tex <==
\begin{figure}[tb]
  \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{sec/figs/sec3_method/arbitrary_scale.pdf}

   \caption{Text-driven arbitrary-scale super-resolution. Besides degradation-blind restoration, our method support conditioning from natural language through CLIP, which is different from previous work that conditioned on a floating-point rescaling factor,}
   \label{fig:arbitray-scale-sr}
\end{figure}

==> sec/figs/sec4_exp/ablation_study.tex <==
\begin{table*}[!t]
\centering
% \centeringbat
\setlength{\tabcolsep}{1.6pt}
\renewcommand{\arraystretch}{1.0}

\begin{tabular} 
{@{}l@{\hspace{2mm}}*{4}{c@{\hspace{3mm}}}c@{\hspace{1mm}}r@{}}
% \hline
% \rowcolor[gray]{0.95}
\toprule
Method & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & \small{CLIP-image}$\uparrow$ & \small{CLIP-text}$\uparrow$ \\
\midrule

Ours ControlNet with text~\cite{zhang2023controlnet} & 12.135 & 0.223 & 23.50 & 0.660 & 0.940 & \textbf{0.306}\\
Ours trained w/o enhance param "deblur, denoise"& 11.577 & 0.223 & 23.61 & 0.665 & 0.942 & 0.305 \\\hline

Ours-full & \textbf{11.343} & \textbf{0.219} & 23.61 & 0.665 & \textbf{0.943} & 0.305\\

\end{tabular}

\caption{Ablation study}
\label{tab:main-table}

\end{table*}

==> sec/figs/sec4_exp/main_visuals_sep.tex <==
% \begin{figure*}[t]
%   \centering
% %   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=0.99\linewidth,height=0.4\linewidth]{example-image-golden}
%   \caption{Main visual results.}
%   \label{fig:main-visuals}
% \end{figure*}


% lumascope links of following result: https://brook-cycle-730.notion.site/visual-comparison-5935df26e84e42a689245fa0fde90cf2?pvs=4

% A backup version is in x_suppl.tex

\newcommand{\imgwidth}{0.4\columnwidth}

\begin{figure*}[t]
\centering
% \footnotesize
\setlength\tabcolsep{1pt}
{
\renewcommand{\arraystretch}{0.6}
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}*{7}{c}@{}}
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_lr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_diffbir.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_diffbir_sdedit.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_diffbir_prompt.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_ours_wo_prompt.jpg} 
     & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_ours.jpg} & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_hr.jpg}\\
     \multicolumn{7}{c}{\emrph{A blue, white and red fire hydrant sitting on a sidewalk}} \\
     
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/3_young_giraffes/002401_lr.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/3_young_giraffes/002401_diffbir.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/3_young_giraffes/002401_diffbir_sdedit.jpg} &
      \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/3_young_giraffes/002401_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/3_young_giraffes/002401_ours_wo_prompt.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/3_young_giraffes/002401_ours.jpg} 
    %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_ours.jpg} 
     & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/3_young_giraffes/002401_hr.jpg}\\
     \multicolumn{7}{c}{\emrph{Four young giraffes in a zoo, with one of them being fed leaves by a person}} \\

    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/4_bus_cow/002050_lr.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/4_bus_cow/002050_diffbir.jpg} & 
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/4_bus_cow/002050_diffbir_sdedit.jpg} &
    %   \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/4_bus_cow/002050_diffbir_prompt.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/4_bus_cow/002050_ours_wo_prompt.jpg} & 
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/4_bus_cow/002050_ours.jpg} 
    % %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_ours.jpg} 
    %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/4_bus_cow/002050_hr.jpg}\\   

    %  \multicolumn{7}{c}{\emrph{A group of cows on street next to building and bus.}} \\

     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/5_hands_phone/002578_lr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/5_hands_phone/002578_diffbir.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/5_hands_phone/002578_diffbir_sdedit.jpg} &
      \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/5_hands_phone/002578_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/5_hands_phone/002578_ours_wo_prompt.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/5_hands_phone/002578_ours.jpg} 
    %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_ours.jpg} 
     & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/5_hands_phone/002578_hr.jpg}\\ 
     \multicolumn{7}{c}{\emrph{Two hands holding and dialing a cellular phone.}} \\

     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/6_boat/002108_lr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/6_boat/002108_diffbir.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/6_boat/002108_diffbir_sdedit.jpg} &
      \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/6_boat/002108_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/6_boat/002108_our_wo_text.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/6_boat/002108_ours.jpg} 
    %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_ours.jpg} 
     & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/6_boat/002108_hr.jpg}\\ 
     \multicolumn{7}{c}{\emrph{An old boat sitting in th emiddle of a field.}} \\

    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/7_zebra/001102_lr.jpg} & 
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/7_zebra/001102_diffbir.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/7_zebra/001102_diffbir_sdedit.jpg} &
    %   \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/7_zebra/001102_diffbir_prompt.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/7_zebra/001102_ours_wo_prompt.jpg} & 
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/7_zebra/001102_ours.jpg} 
    % %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_ours.jpg} 
    %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/7_zebra/001102_hr.jpg}\\ 

    %  \multicolumn{7}{c}{\emrph{Zebras crossing a bitumen road in the savannah.}} \\

    %   & & & & \\
     input & DiffBIR~\cite{Lin2023diffbir} & DiffBIR + SDEdit~\cite{sdedit} & DiffBIR + Cont. Prompt &
     Ours w/o Cont. Prompt & Ours Full Model & Ground-Truth
\end{tabular}
}
}
\caption{Main visual results.}
\label{fig:main-visuals}
\end{figure*}





\begin{figure*}[t]
\centering
% \footnotesize
\setlength\tabcolsep{1pt}
{
\renewcommand{\arraystretch}{0.6}
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}*{7}{c}@{}}
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/8_train/000014_lr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/8_train/000014_diffbir.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/8_train/000014_diffbir_sdedit.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/8_train/000014_diffbir_prompt.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/8_train/000014_ours_wo_text.jpg} 
     & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/8_train/000014_ours.jpg} & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/8_train/000014_hr.jpg}\\
     \multicolumn{7}{c}{\emrph{A gray train riding on a track.}} \\
     
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/9_zebra/000058_lr.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/9_zebra/000058_diffbir.jpg} & 
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/9_zebra/000058_diffbir_sdedit.jpg} &
    %   \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/9_zebra/000058_diffbir_prompt.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/9_zebra/000058_ours_wo_prompt.jpg} & 
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/9_zebra/000058_ours.jpg} 
    % %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_ours.jpg} 
    %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/9_zebra/000058_hr.jpg}\\
    %  \multicolumn{7}{c}{\emrph{Two zebras are heading into the bushes as another is heading in the opposite direction.}} \\

    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/10_street_cars/000050_lr.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/10_street_cars/000050_diffbir.jpg} & 
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/10_street_cars/000050_sdedit.jpg} &
    %   \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/10_street_cars/000050_diffbir_prompt.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/10_street_cars/000050_ours_wo_prompt.jpg} & 
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/10_street_cars/000050_ours.jpg} 
    % %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_ours.jpg} 
    %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/10_street_cars/000050_hr.jpg}\\   

    %  \multicolumn{7}{c}{\emrph{A street with cars and construction workers working.}} \\

     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/11_sign_leaves/000053_lr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/11_sign_leaves/000053_diffbir.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/11_sign_leaves/000053_diffbir_sdedit.jpg} &
      \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/11_sign_leaves/000053_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/11_sign_leaves/000053_ours_wo_prompt.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/11_sign_leaves/000053_ours.jpg} 
    %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_ours.jpg} 
     & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/11_sign_leaves/000053_hr.jpg}\\ 
     \multicolumn{7}{c}{\emrph{A street sign surrounded by orange and red leaves.}} \\

     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/12_giraffes/000172_lr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/12_giraffes/000172_diffbir.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/12_giraffes/000172_diffbir_sdedit.jpg} &
      \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/12_giraffes/000172_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/12_giraffes/000172_ours_wo_prompt.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/12_giraffes/000172_ours.jpg} 
    %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_ours.jpg} 
     & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/12_giraffes/000172_hr.jpg}\\ 
     \multicolumn{7}{c}{\emrph{Two giraffes are standing together outside near a wall.}} \\

     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/13_bird/000091_lr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/13_bird/000091_diffbir.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/13_bird/000091_diffbir_sdedit.jpg} &
      \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/13_bird/000091_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/13_bird/000091_ours_wo_prompt.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/13_bird/000091_ours.jpg}  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/13_bird/000091_hr.jpg}\\ 

     \multicolumn{7}{c}{\emrph{A bird is sitting on a branch among unfocused trees.}} \\

     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/14_bears_rocks/000136_lr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/14_bears_rocks/000136_diffbir.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/14_bears_rocks/000136_diffbir_sdedit.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/14_bears_rocks/000136_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/14_bears_rocks/000136_ours_wo_text.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/14_bears_rocks/000136_ours.jpg}  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/14_bears_rocks/000136_hr.jpg}\\ 

     \multicolumn{7}{c}{\emrph{two brown bears on some rocks.}} \\

    %   & & & & \\
     input & DiffBIR~\cite{Lin2023diffbir} & DiffBIR + SDEdit~\cite{sdedit} & DiffBIR + Cont. Prompt &
     Ours w/o Cont. Prompt & Ours Full Model & Ground-Truth
\end{tabular}
}
}
\caption{Main visual results on Real-Esrgan Degradation pipeline.}
\label{fig:main-visuals-resrgan}
\end{figure*}



==> sec/figs/sec4_exp/main_visuals_supp1.tex <==
\newcommand{\imgwidth}{0.4\columnwidth}

\begin{figure*}[t]
\centering
% \footnotesize
\setlength\tabcolsep{1pt}
{
\renewcommand{\arraystretch}{0.6}
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}*{7}{c}@{}}
     Input & DiffBIR~\cite{Lin2023diffbir} & DiffBIR + SDEdit~\cite{sdedit} & DiffBIR + CLIP~\cite{radford2021clip} & ControlNet-SR~\cite{luo2023controlling} & Ours TIP Model & Ground-Truth \\
    
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/2_giraffe_eating/002552_lr.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/2_giraffe_eating/002552_diffbir.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/2_giraffe_eating/002552_diffbir_sdedit.jpg} &
      \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/2_giraffe_eating/002552_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/2_giraffe_eating/002552_ours_without_text.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/2_giraffe_eating/002552_ours.jpg} 

     & \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/2_giraffe_eating/002552_hr.jpg}\\
     
     \multicolumn{7}{c}{\emph{A tall giraffe eating leafy greens in a jungle.}} \\
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/4_bus_cow/002050_lr.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/4_bus_cow/002050_diffbir.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/4_bus_cow/002050_diffbir_sdedit.jpg} &
      \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/4_bus_cow/002050_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/4_bus_cow/002050_ours_wo_prompt.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/4_bus_cow/002050_ours.jpg} 
     & \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/4_bus_cow/002050_hr.jpg}\\   

     \multicolumn{7}{c}{\emph{A group of cows on street next to building and bus.}} \\


     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/7_zebra/001102_lr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/7_zebra/001102_diffbir.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/7_zebra/001102_diffbir_sdedit.jpg} &
      \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/7_zebra/001102_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/7_zebra/001102_ours_wo_prompt.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/7_zebra/001102_ours.jpg} 
     & \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/7_zebra/001102_hr.jpg}\\ 

     \multicolumn{7}{c}{\emph{Zebras crossing a bitumen road in the savannah.}} \\

    %   & & & & \\

\end{tabular}
}
}
\caption{More visual comparisons.}
\label{fig:main-visuals-supp1}
\end{figure*}


==> sec/figs/sec4_exp/main_visuals_supp2.tex <==

\newcommand{\imgwidth}{0.4\columnwidth}

\begin{figure*}[t]
\centering
% \footnotesize
\setlength\tabcolsep{1pt}
{
\renewcommand{\arraystretch}{0.6}
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}*{7}{c}@{}}
     Input & DiffBIR~\cite{Lin2023diffbir} & DiffBIR + SDEdit~\cite{sdedit} & DiffBIR + CLIP~\cite{radford2021clip} & ControlNet-SR~\cite{luo2023controlling} & Ours TIP Model & Ground-Truth \\
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/8_train/000014_lr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/8_train/000014_diffbir.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/8_train/000014_diffbir_sdedit.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/8_train/000014_diffbir_prompt.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/8_train/000014_ours_wo_text.jpg} 
     & \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/8_train/000014_ours.jpg} & \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/8_train/000014_hr.jpg}\\
     \multicolumn{7}{c}{\emph{A gray train riding on a track.}} \\
     
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/9_zebra/000058_lr.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/9_zebra/000058_diffbir.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/9_zebra/000058_diffbir_sdedit.jpg} &
      \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/9_zebra/000058_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/9_zebra/000058_ours_wo_prompt.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/9_zebra/000058_ours.jpg} 
    %  & \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/1_hydrant/000967_ours.jpg} 
     & \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/9_zebra/000058_hr.jpg}\\
     \multicolumn{7}{c}{\emph{Two zebras are heading into the bushes as another is heading in the opposite direction.}} \\
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/10_street_cars/000050_lr.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/10_street_cars/000050_diffbir.jpg} & 
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/10_street_cars/000050_sdedit.jpg} &
    %   \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/10_street_cars/000050_diffbir_prompt.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/10_street_cars/000050_ours_wo_prompt.jpg} & 
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/10_street_cars/000050_ours.jpg} 
    % %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/1_hydrant/000967_ours.jpg} 
    %  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/10_street_cars/000050_hr.jpg}\\   

    % %  \multicolumn{7}{c}{\emph{A STREET WITH CARS AND CONSTRUCTION WORKERS WORKING.}} 
    %  \multicolumn{7}{c}{\emph{A street with cars and construction workers working.}} \\

     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/11_sign_leaves/000053_lr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/11_sign_leaves/000053_diffbir.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/11_sign_leaves/000053_diffbir_sdedit.jpg} &
      \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/11_sign_leaves/000053_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/11_sign_leaves/000053_ours_wo_prompt.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/11_sign_leaves/000053_ours.jpg} 
    %  & \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/1_hydrant/000967_ours.jpg} 
     & \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/11_sign_leaves/000053_hr.jpg}\\ 
     \multicolumn{7}{c}{\emph{A street sign surrounded by orange and red leaves.}} \\

     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/12_giraffes/000172_lr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/12_giraffes/000172_diffbir.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/12_giraffes/000172_diffbir_sdedit.jpg} &
      \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/12_giraffes/000172_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/12_giraffes/000172_ours_wo_prompt.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/12_giraffes/000172_ours.jpg} 
    %  & \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/1_hydrant/000967_ours.jpg} 
     & \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/12_giraffes/000172_hr.jpg}\\ 
     \multicolumn{7}{c}{\emph{Two giraffes are standing together outside near a wall.}} \\

    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/13_bird/000091_lr.jpg} & 
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/13_bird/000091_diffbir.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/13_bird/000091_diffbir_sdedit.jpg} &
    %   \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/13_bird/000091_diffbir_prompt.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/13_bird/000091_ours_wo_prompt.jpg} & 
    %  \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/13_bird/000091_ours.jpg}  & \includegraphics[width=\imgwidth]{sec/figs/sec4_exp/13_bird/000091_hr.jpg}\\ 

    %  \multicolumn{7}{c}{\emph{A bird is sitting on a branch among unfocused trees.}} \\

     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/14_bears_rocks/000136_lr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/14_bears_rocks/000136_diffbir.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/14_bears_rocks/000136_diffbir_sdedit.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/14_bears_rocks/000136_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/14_bears_rocks/000136_ours_wo_text.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/14_bears_rocks/000136_ours.jpg}  & \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/14_bears_rocks/000136_hr.jpg}\\ 

     \multicolumn{7}{c}{\emph{two brown bears on some rocks.}} \\

    %  \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/15_tennis_player/000246_lr.jpg} & 
    %  \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/15_tennis_player/000246_diffbir.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/15_tennis_player/000246_diffbir_sdedit.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/15_tennis_player/000246_diffbir_prompt.jpg} &
    %  \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/15_tennis_player/000246_ours_wo_prompt.jpg} & 
    %  \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/15_tennis_player/000246_ours.jpg}  & \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/15_tennis_player/000246_hr.jpg}\\ 

    %  \multicolumn{7}{c}{\emph{There is a female tennis player.}} \\

     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/16_stop_sign/000362_lr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/16_stop_sign/000362_diffbir.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/16_stop_sign/000362_diffbir_sdedit.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/16_stop_sign/000362_diffbir_prompt.jpg} &
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/16_stop_sign/000362_controlnetsr.jpg} & 
     \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/16_stop_sign/000362_ours.jpg}  & \includegraphics[width=\imgwidth]{sec/figs/supp/crop_result/16_stop_sign/000362_hr.jpg}\\ 

     \multicolumn{7}{c}{\emph{A stop sign with graffiti on it nailed to a pole.}} \\

    %   & & & & \\
    %  input & DiffBIR~\cite{Lin2023diffbir} & DiffBIR + SDEdit~\cite{sdedit} & DiffBIR + Cont. Prompt &
    %  Ours w/o Cont. Prompt & Ours Full Model & Ground-Truth
\end{tabular}
}
}
\caption{Main visual results on Real-Esrgan Degradation pipeline.}
\label{fig:main-visuals-supp2}
\end{figure*}


==> sec/tabs/breakdown.tex <==
\begin{table*}[!t]
\centering
% \centeringbat
\setlength{\tabcolsep}{1.6pt}
\renewcommand{\arraystretch}{1.0}

\begin{tabular} 
{@{}l@{\hspace{2mm}}*{5}{c@{\hspace{2mm}}}r@{}}
% \hline
% \rowcolor[gray]{0.95}
\toprule
Method & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\downarrow$ & LPIPS$\downarrow$ & CLIP-image $\downarrow$ & CLIP-text $\downarrow$ \\
\midrule
% \textcolor{blue}{$\bullet$}NIMA~\cite{talebi2018nima} & $224$ & 56M & 0.636  \\
% \textcolor{blue}{$\bullet$}+\cite{talebi2021learning}$_{512\rightarrow 224}$ & $224$ & 56M & 0.680 \\
% \textcolor{blue}{$\bullet$}EffNet-B0~\cite{tan2019efficientnet} & $224$ & 5.3M & 0.642 \\
% \textcolor{blue}{$\bullet$}+\cite{talebi2021learning}$_{512\rightarrow 224}$ & $224$ & 5.3M & 0.650 \\
% Real-ESRGAN
% Real-ESRGAN
% \textit{Regression-based} \\ \hdashline
% \textit{GAN-based} \\ \hdashline
Real-ESRGAN~\cite{wang2021real-esrgan} & \\
SwinIR~\cite{} \\
DiffIR~\cite{} \\
DiffBIR~\cite{Lin2023diffbir} &  \\
StableSR~\cite{wang2023stablesr} & 20.551 & 0.313 \\
StableSR (w/ cont prompt)~\cite{wang2023stablesr} & 20.551 & 0.313 \\\hline

Ours ControlNet~\cite{zhang2023controlnet} & 12.135 & 0.223\\
Ours w/o text & 13.649 & 0.222\\
Ours w/o $\text{text}_{enhance}$ & 11.710 & 0.226 \\
%\textcolor{red}{$\circ$}MUSIQ~\cite{ke2021musiq} & Full-res & 27M & 0.731 & \textbf{0.719} \\\hline
Ours w/o enhance param & 11.577 & 0.223 \\\hline
Ours & \textbf{11.343} & \textbf{0.219} \\
Ours-blind & & 
%\textcolor{green}{$\diamond$}MaxViT-T & $384$ & 31M & 0.736 & 0.699 \\
%\textcolor{green}{$\diamond$}MaxViT-T & $512$ & 31M & \textbf{0.745} & \textbf{0.708} \\
% \bottomrule
\end{tabular}
\caption{Task break-down experiments}
\label{tab:main-table}
% \vspace{-3mm}
\end{table*}

==> sec/tabs/rebuttal_blined_restoration.tex <==
% % \vspace{-1em}
% \begin{table}[h]
% \centering
% % \centeringbat
% \setlength{\tabcolsep}{1.6pt}
% \renewcommand{\arraystretch}{1.0}
% \resizebox{0.8\linewidth}{!}{
% \begin{tabular} 
% {@{}l@{\hspace{2mm}}*{4}{c@{\hspace{3mm}}}c@{\hspace{1mm}}r@{}}
% \vspace{-1em}
% \toprule
% % \multicolumn{1}{l}{} & \multicolumn{2}{c}{Parameterized Degradation} & & \multicolumn{2}{c}{Real-ESRGAN Degradation }
% % \cmidrule(l{0mm}r{1mm}){2-3} 
% % &
% % \cmidrule(l{1mm}r{1mm}){2-3}
% % \cmidrule(l{1mm}r{0mm}){4-5}
% Method without restoration prompts & FID$\downarrow$ & LPIPS$\downarrow$ &  & FID & LPIPS
% \\
% \midrule

% Ours without semantic prompt \\
% % & 0.300\\
% Ours with semantic prompt \\ 
% % \textbf{0.273}\\
% % Ours w/o text (finetuned) & \\
% % & \textbf{0.30} \\
% % Ours tested w/o text & \\
% \bottomrule
% \end{tabular}
% }
% \vspace{-1ex}
% % \caption{ \todo{semantic prompt for blind }. }
% % \label{tab:other_testset}
% \vspace{-1em}
% \end{table}



\begin{table}[h]
\centering
% \centeringbat
\setlength{\tabcolsep}{1.6pt}
\renewcommand{\arraystretch}{1.0}
\vspace{-0.35cm}
\resizebox{\linewidth}{!}{
\begin{tabular} 
{@{}l@{\hspace{2mm}}*{4}{c@{\hspace{3mm}}}c@{\hspace{1mm}}r@{}}
% \hline
% \rowcolor[gray]{0.95}
\toprule
% Method & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & \small{CLIP-image}$\uparrow$ & \small{CLIP-text}$\uparrow$ \\
% & \multicolumn{4}{c}{DIV2K-Val} \\
% & \multicolumn{1}{c}{RealSRSet} \\
% \cmidrule(l{1mm}r{1mm}){2-5} 
% \cmidrule(l{1mm}r{1mm}){6-6}
% Method & FID$\downarrow$ & LPIPS$\downarrow$ & Params & FLOPs & inference speed & Timestep & 
%  & \multicolumn{2}{l}{Parameterized Degradation} & & \multicolumn{2}{l}{Real-ESRGAN Degradation } 
%  \\
Method without restoration prompts & FID$\downarrow$ & CLIP-I$\uparrow$ & CLIP-T$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$
% PSNR$\uparrow$ & SSIM$\uparrow$ &
% \small{CLIP\textsubscript{image}}$\uparrow$ & LPIPS$\downarrow$ &
% \small{CLIP-I}$\uparrow$ 
% & LPIPS$\downarrow$
\\
% \cmidrule(l{1mm}r{1mm}){10-15}
\midrule
Ours without semantic prompt & 13.60 &  0.939 & 0.300 & \textbf{0.221} & \textbf{23.65} \\
Ours with semantic prompt & \textbf{11.71} &  \textbf{0.941} & \textbf{0.305} & {0.226} & 23.55 \\
\bottomrule
\end{tabular}
}
% \vspace{-1em}
% \caption{\todo{Comparison of computation cost}. }
% \label{tab:other_testset}
\vspace{-1em}
\end{table}


==> sec/tabs/rebuttal_computation.tex <==

\begin{table}[h]
\centering
% \centeringbat
\setlength{\tabcolsep}{1.6pt}
\renewcommand{\arraystretch}{1.0}
\vspace{-0.35cm}
\resizebox{0.98\linewidth}{!}{
\begin{tabular} 
{@{}l@{\hspace{2mm}}*{4}{c@{\hspace{3mm}}}c@{\hspace{1mm}}r@{}}
% \hline
% \rowcolor[gray]{0.95}
\toprule
% Method & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & \small{CLIP-image}$\uparrow$ & \small{CLIP-text}$\uparrow$ \\
% & \multicolumn{4}{c}{DIV2K-Val} \\
% & \multicolumn{1}{c}{RealSRSet} \\
% \cmidrule(l{1mm}r{1mm}){2-5} 
% \cmidrule(l{1mm}r{1mm}){6-6}
\todo{Method consider remove this} & FID$\downarrow$ & LPIPS$\downarrow$ & Params & FLOPs & inference speed & Timestep
% PSNR$\uparrow$ & SSIM$\uparrow$ &
% \small{CLIP\textsubscript{image}}$\uparrow$ & LPIPS$\downarrow$ &
% \small{CLIP-I}$\uparrow$ 
% & LPIPS$\downarrow$
\\
% \cmidrule(l{1mm}r{1mm}){10-15}
\midrule
DiffBIR (zero-shot) &  \\
% & ~\\
%  DiffBIR~\cite{Lin2023diffbir} + SDEdit~\cite{sdedit} &  \\
StableSR &  \\
% & 0.300\\
Ours &. \\
% \textbf{0.273}\\
% Ours w/o text (finetuned) & \\
% & \textbf{0.30} \\
% Ours tested w/o text & \\
\bottomrule
\end{tabular}
}
\vspace{-0.5em}
% \caption{\todo{Comparison of computation cost}. }
% \label{tab:other_testset}
% \vspace{-1em}
\end{table}



==> sec/tabs/rebuttal_degradation_pipeline.tex <==
\begin{table}[h]
\centering
\setlength{\tabcolsep}{1.6pt}
\renewcommand{\arraystretch}{1.0}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l@{\hspace{3mm}}crl}
% \toprule
Degradation Process &  Restoration Prompt & range of hyperparameter
\\
% \midrule
\toprule
Gaussian Blur  & Deblur with \{sigma\}  & [0.2, 3.0]
\\
Downsample    & Upsample to \{resizing factor\}  & [1.0, 7.0]
\\
Gaussian Noise  & Denoise with \{sigma\}  & [0.0, 0.12]
\\
JPEG           & Dejpeg with quality \{jpeg quality\}  & [30, 92]
\\
\bottomrule
\end{tabular}
}
\label{tab:Degradation_pipeline}
\end{table}



==> sec/tabs/rebuttal_div2k_comparison.tex <==




\begin{table}[t]
\centering
\scriptsize
% \resizebox{\linewidth}{!}
{
\begin{tabular} 
{@{}l@{\hspace{2mm}}*{4}{c@{\hspace{3mm}}}c@{\hspace{1mm}}r@{}}
% \vspace{1mm}
% \toprule
% \hline

Method & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ &

\small{CLIP-I}$\uparrow$ &
\small{CLIP-T}$\uparrow$ 

\\

% \midrule
% \hline
\toprule


Real-ESRGAN  & 32.37 & 0.312 & 22.52 & \textbf{0.646} & 0.683 & \textbf{0.325}  \\
Ours  & \textbf{14.42} & \textbf{0.262} & 
\textbf{23.14} & 0.633 & \textbf{0.935} & 0.308
\\

\bottomrule
% \hline
\end{tabular}

}
\caption{Comparison with Real-ESRGAN on DIV2k with Real-ESRGAN degradation.}
  \label{tab:other_testset}

\end{table}


==> sec/tabs/rebuttal_running_cost.tex <==
\begin{table}[h]
\centering
\setlength{\tabcolsep}{1.6pt}
\renewcommand{\arraystretch}{1.0}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l@{\hspace{3mm}}crl}
\toprule
Model &  speed & parameters & GFLOPS
\\
\midrule
Ours  & 1.4s (50 timesteps on TPU)  & 1130 per step
\\
StableSR    & Upsample to \{resizing factor\}  & [1.0, 7.0]
\\
DiffBir  & Denoise with \{sigma\}  & [0.0, 0.12]
\\
% JPEG           & Dejpeg with quality \{jpeg quality\} or Dejpeg & [30, 92]
\\
\bottomrule
\end{tabular}
}
\label{tab:Degradation_pipeline}
\end{table}


